Model-Value Inconsistency as a Signal for Epistemic Uncertainty

Using a model of the environment and a value function, an agent can construct many estimates of a state's value, by unrolling the model for different lengths and bootstrapping with its value function. Our key insight is that one can treat this set of value estimates as a type of ensemble, which we call an \emph{implicit value ensemble} (IVE). Consequently, the discrepancy between these estimates can be used as a proxy for the agent's epistemic uncertainty; we term this signal \emph{model-value inconsistency} or \emph{self-inconsistency} for short. Unlike prior work which estimates uncertainty by training an ensemble of many models and/or value functions, this approach requires only the single model and value function which are already being learned in most model-based reinforcement learning algorithms. We provide empirical evidence in both tabular and function approximation settings from pixels that self-inconsistency is useful (i) as a signal for exploration, (ii) for acting safely under distribution shifts, and (iii) for robustifying value-based planning with a learned model.

==> figures/ive_computation.tex <==
\begin{figure*}[t]
  \centering
  \begin{subfigure}[b]{\linewidth}
    \centering
    \input{assets/tikz/ive_muesli_cge}
    % \caption{Computation graph for the generation of n }
    % \label{subfig:vensemble-net}
  \end{subfigure}
  \caption{
    Computation graph for the generation of the n members of \emph{Implicit Value Emsemble}, with each MVP being generated through sequential model unrolls. Each IVE member computes a different trade-off between value and reward predictions.
  }
  \label{fig:ive-muesli-cg}
\end{figure*}

==> figures/muesli-planning.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.3\linewidth]{assets/procgen/planning_plot_SE_leg.pdf}
    \includegraphics[width=\linewidth]{assets/procgen/planning_plot_SE.pdf}
    \caption{
    Muesli experiments on ProcGen environments, where the ensemble average, i.e., $\mu$-IVE(5) or single ensemble members. i.e., $\vhat_{\mhat}^{1}$ and $\vhat_{\mhat}^{5}$, are used for value prediction.
    Lines show mean episodic returns over 100 training levels and error bars show standard error across 3 seeds.
    }
    \label{fig:muesli-planning}
\end{figure*}
